ParetoPrep: Fast computation of Path Skylines Queries

Computing cost optimal paths in network data is a very important task in many application areas like transportation networks, computer networks or social graphs. In many cases, the cost of an edge can be described by various cost criteria. For example, in a road network possible cost criteria are distance, time, ascent, energy consumption or toll fees. In such a multicriteria network, a route or path skyline query computes the set of all paths having pareto optimal costs, i.e. each result path is optimal for different user preferences. In this paper, we propose a new method for computing route skylines which significantly decreases processing time and memory consumption. Furthermore, our method does not rely on any precomputation or indexing method and thus, it is suitable for dynamically changing edge costs. Our experiments demonstrate that our method outperforms state of the art approaches and allows highly efficient path skyline computation without any preprocessing.

==> graphic_algorithmexecution.tex <==
\tikzstyle{closed}=[circle, draw=black, minimum size = 8mm, thick, node distance = 12mm]
\tikzstyle{open}=[circle, fill=gray!25, draw=black, minimum size = 8mm, thick, node distance = 12mm]
%\tikzstyle{cost}=[rectangle, draw=black!20, minimum size = 5mm, thin, node distance = 10mm]
\tikzstyle{cost}=[rectangle, draw=black!20, minimum size = 5mm, thin, node distance = 10mm]
\tikzstyle{edge}=[]
\tikzstyle{arc}=[->,dashed]
\tikzstyle{pred}=[thin, ->]
\tikzstyle{pred2}=[very thick, ->]
\newcommand{\nodes}[8]{
\node[#1](s){$s$};
\node[#3](n1)[above right of =s, right=0.5]{$n_1$};
\node[#5](n2)[below right of =s, right=0.5]{$n_2$};
\node[#7](d)[below right of = n1, right=0.5]{$t$};
%\node[cost](scost)[left of =s, left=-0.4]{\scriptsize $c(s) = [#2]$};
%\node[cost](n1cost)[above of =n1, above=-0.5]{\scriptsize $c(n_1) =[#4]$};
%\node[cost](n2cost)[below of =n2, below=-0.5]{\scriptsize $c(n_2) = [#6]$};
%\node[cost](dcost)[right of =d, right=-0.4]{ \scriptsize $c(dest) = [#8]$};

\node[cost](scost)[left of =s, left=-0.35]{\scriptsize $lb(s) = [#2]$};
\node[cost](n1cost)[above of =n1, above=-0.5]{\scriptsize $lb(n_1) = [#4]$};
\node[cost](n2cost)[below of =n2, below=-0.5]{\scriptsize $lb(n_2) = [#6]$};
\node[cost](dcost)[right of =d, right=-0.35]{ \scriptsize $lb(t) = [#8]$};
\node(dummy)[above of =n1cost, above=-0.7]{};
}
\newcommand{\iteration}[2]{
\node[](s)[left of=n1cost, left=0.5]{#1};
\node[](s)[right of=n1cost,right=0.5]{$open = \{#2\}$};
}
\newcommand{\arcsm}[6]{
\path 
(s) edge [#1, bend left=25] node[edge, above=0.1] {\scriptsize $[2,1]$} (n1)
(s) edge [#2, bend right=25] node[edge, below=0.1] {\scriptsize $[3,3]$} (n2)
(n1) edge [#3, bend right=25] node[edge, left=0.05] {\scriptsize $[1,1]$} (n2);
\path
(n2) edge [#4, bend right=25] node[edge, right=0.05] {\scriptsize $[1,1]$} (n1)
(n1) edge [#5, bend left=25] node[edge, above=0.1] {\scriptsize $[1,3]$} (d)
(n2) edge [#6, bend right=25] node[edge, below=0.1] {\scriptsize $[3,1]$} (d)
;
}
%\newcommand{\iteration}[2]{\scriptsize $$\text{#1: } open = \{ #2 \} $$} 
\begin{tikzpicture}[scale=0.9, transform shape]
\nodes{closed}{\infty,\infty}{closed}{\infty,\infty}{closed}{\infty,\infty}{open}{0,0}
\arcsm{arc}{arc}{arc}{arc}{arc}{arc}
\iteration{Iteration 1}{\underline{t}}
\end{tikzpicture}

\begin{tikzpicture}[scale=0.9, transform shape]
\nodes{closed}{\infty,\infty}{open}{\textbf{1,3}}{open}{\textbf{3,1}}{closed}{0,0}
\arcsm{arc}{arc}{arc}{arc}{pred}{pred}
\iteration{Iteration 2}{\underline{n_1}, n_2}
\end{tikzpicture}
%$$ pred(n_1) = \{ arc(n_1, dest) \} $$
%$$ pred(n_2) = \{ arc(n_2, dest) \} $$
%\scriptsize $$ open = \{ n_1 \} $$

\begin{tikzpicture}[scale=0.9, transform shape]
\nodes{closed}{3,4}{closed}{1,3}{open}{\textbf{2},1}{closed}{0,0}
\arcsm{pred2}{arc}{arc}{pred}{pred2}{pred}
\iteration{Iteration 3}{\underline{n_2}}
\end{tikzpicture}

%\scriptsize $$ open = \{ n_2 \} $$
\begin{tikzpicture}[scale=0.9, transform shape]
\nodes{closed}{3,4}{open}{1,\textbf{2}}{closed}{2,1}{closed}{0,0}
\arcsm{pred2}{pred}{pred}{pred}{pred2}{pred}
\iteration{Iteration 4}{\underline{n_1}}
\end{tikzpicture}

%\scriptsize $$ open = \{ \} $$
\begin{tikzpicture}[scale=0.9, transform shape]
\nodes{closed}{3,\textbf{3}}{closed}{1,2}{closed}{2,1}{closed}{0,0}
\arcsm{pred2}{pred}{pred2}{pred}{pred2}{pred2}
\iteration{Termination}{}
\end{tikzpicture}

==> graphic_domination.tex <==
\begin{tikzpicture}[transform shape,scale=0.75]

\coordinate (o) at (0, 0);
\coordinate (x) at (6, 0);
\coordinate (y) at (0, 6.5);

\coordinate (a) at (0.5, 4.5);
\coordinate (b) at (1.5, 3.5);
\coordinate (c) at (2.5, 3);
\coordinate (d) at (2.75, 1.5);
\coordinate (e) at (1, 5.5);
\coordinate (f) at (3.5, 4);
\coordinate (g) at (4, 1.5);
\coordinate (h) at (5, 6);

\draw[fill=black!7, draw=none] (0.5,6.5) -- (a) -- (1.5,4.5) -- (b) -- (2.5,3.5) -- (c) -- (2.75,3) -- (d) -- (6,1.5) -- (6,6.5) -- cycle;
\draw[ very thin, draw=black!50] (0.5,6.5) -- (a) -- (1.5,4.5) -- (b) -- (2.5,3.5) -- (c) -- (2.75,3) -- (d) -- (6,1.5);

\node at (x) [right=0.1]{first cost};
\node at (y) [above=0.1]{second cost};

\draw[fill=white,draw=black] (a) circle(2pt);
\node at (a) [below=0.1]{$a$};

\draw[fill=white,draw=black] (b) circle(2pt);
\node at (b) [below=0.1]{$b$};

\draw[fill=white,draw=black] (c) circle(2pt);
\node at (c) [below=0.1]{$c$};

\draw[fill=white,draw=black] (d) circle(2pt);
\node at (d) [below=0.1]{$d$};

\draw[fill=black,draw=black] (e) circle(2pt);
\node at (e) [below=0.1]{$e$};
%\node at (e) [below right]{\,(dominated by $a$)};

\draw[fill=black,draw=black] (f) circle(2pt);
\node at (f) [below=0.1]{$f$};
%\node at (f) [below right]{\ (dominated by $b$, $c$ and $d$)};

\draw[fill=black,draw=black] (g) circle(2pt);
\node at (g) [below=0.15]{$g$}; 
%\node at (g) [below right]{\,(dominated by $d$)};

\draw[fill=black,draw=black] (h) circle(2pt);
\node at (h) [below=0.05]{$h$};
%\node at (h) [below right=0.05]{(dominated by all)};

\draw[thick, ->] (o) -- (x);
\draw[thick, ->] (o) -- (y);
\end{tikzpicture}

